The Semantics of Rank Polymorphism

Iverson's APL and its descendants (such as J, K and FISh) are examples of the family of "rank-polymorphic" programming languages. The principal control mechanism of such languages is the general lifting of functions that operate on arrays of rank (or dimension) $r$ to operate on arrays of any higher rank $r' > r$. We present a core, functional language, Remora, that captures this mechanism, and develop both a formal, dynamic semantics for the language, and an accompanying static, rank-polymorphic type system for the language. Critically, the static semantics captures the shape-based lifting mechanism of the language. We establish the usual progress and preservation properties for the type system, showing that it is sound, which means that "array shape" errors cannot occur at run time in a well-typed program. Our type system uses dependent types, including an existential type abstraction which permits programs to operate on arrays whose shape or rank is computed dynamically; however, it is restricted enough to permit static type checking. The rank-polymorphic computational paradigm is unusual in that the types of arguments affect the dynamic execution of the program -- they are what drive the rank-polymorphic distribution of a function across arrays of higher rank. To highlight this property, we additionally present a dynamic semantics for a partially erased variant of the fully-typed language and show that a computation performed with a fully-typed term stays in lock step with the computation performed with its partially erased term. The residual types thus precisely characterise the type information that is needed by the dynamic semantics, a property useful for the (eventual) construction of efficient compilers for rank-polymorphic languages.

==> Makefile <==
.SUFFIXES: .pdf .ps $(.SUFFIXES)
.PHONY: all clean realclean bib

all: paper.pdf tutorial.pdf

# Crowbar TEXINPUTS to use *only* packages in this dir and standard packages.
# That way we know the paper will build in a portable way -- no non-standard
# external dependencies.
export TEXINPUTS
TEXINPUTS=.:./texlib//:./inactive//:

# Likewise for BSTINPUTS and bibtex:
export BSTINPUTS
BSTINPUTS=.:./texlib:

BIB = bibtex
PAPERTEX = paper.tex \
	   decls.tex figs.tex \
	   intro.tex tutorial.tex formalism.tex soundness.tex type_erasure.tex

#PAPERSRC = $(PAPERTEX) bib.bib
PAPERSRC = $(PAPERTEX)

paper.pdf: $(PAPERSRC)
tutorial.pdf: tutorial.tex decls.tex

TAGS: $(PAPERSRC)
	etags $^

# Phony targets
###############

# clean: Remove intermediate files, but not final products.
# realclean: Even remove paper.{zip,pdf,ps}.

clean:
	latexmk -c paper.tex
	-rm comment.cut 2>/dev/null || true
#	-rm *.log *.aux *.pdf

realclean: clean
	latexmk -C paper.tex
#	-rm paper.{pdf,dvi,ps} TAGS 2>/dev/null || true

bib:
	$(RUBBER) --clean paper
	latex paper.tex
	$(BIB) paper

# Implicit rules
################

.tex.pdf:
	latexmk -pdf $<
#	pdflatex $<
#	pdflatex $<

.tex.dvi:
	latexmk -dvi $<

.tex.ps:
	latexmk -ps $<



==> decls.tex <==
% Macros used in the paper					% -*- latex -*-

\makeatletter

\newcommand{\ie}{\mbox{\emph{i.e.}}}
\newcommand{\Ie}{\mbox{\emph{I.e.}}}
\newcommand{\eg}{\mbox{\emph{e.g.}}}
\newcommand{\Eg}{\mbox{\emph{E.g.}}}
\newcommand{\etc}{\emph{etc.}}
\newcommand{\nb}{\mbox{\emph{n.b.}}}
\newcommand{\Nb}{\mbox{\emph{N.b.}}}

\newcommand{\sequence}[1]{#1 \, \ldots \,}
\newcommand{\llb}{\left\llbracket}
\newcommand{\rrb}{\right\rrbracket}

\newcommand{\mdoubleplus}{\mathbin{+\mkern-7mu+}}
\newcommand{\thappend}{\mdoubleplus}
\newcommand{\thempty}{\square}
\newcommand{\thprefix}{\sqsubseteq}
\newcommand{\theq}{\equiv}
\providecommand{\dotdiv}{% Don't redefine it if available
  \mathbin{% We want a binary operation
    \vphantom{+}% The same height as a plus or minus
    \text{% Change size in sub/superscripts
      \mathsurround=0pt % To be on the safe side
      \ooalign{% Superimpose the two symbols
        \noalign{\kern-.35ex}% but the dot is raised a bit
        \hidewidth$\smash{\cdot}$\hidewidth\cr % Dot
        \noalign{\kern.35ex}% Backup for vertical alignment
        $-$\cr % Minus
      }}}}
\newcommand{\thmonus}{\dotdiv}

% Syntactic classes
%\newcommand{\scal}{\mathit{s}}
\newcommand{\term}{\mathit{t}}
\newcommand{\atom}{\mathfrak{a}}
\newcommand{\func}{\mathfrak{f}}
\newcommand{\atval}{\mathfrak{v}}
\newcommand{\expr}{\mathit{e}}
\newcommand{\var}{\mathit{x}}
\newcommand{\primop}{\mathfrak{o}}
\newcommand{\val}{\mathit{v}}
\newcommand{\baseval}{\mathfrak{b}}
\newcommand{\type}{\mathit{\tau}}
\newcommand{\basetype}{\mathit{B}}
\newcommand{\kind}{\mathit{k}}
\newcommand{\idx}{\mathit{\iota}}
\newcommand{\sort}{\mathit{\gamma}}
\newcommand{\nat}{\mathit{n}}
\newcommand{\tEnv}{\Gamma}
\newcommand{\kEnv}{\Delta}
\newcommand{\sEnv}{\Theta}
\newcommand{\emptyEnv}{\cdot}
\newcommand{\ctxt}{\mathbb{E}}
\newcommand{\hole}{\square}
\newcommand{\erased}[1]{\widehat{#1}}
\newcommand{\eexpr}{\erased{\expr}}
\newcommand{\eatom}{\erased{\atom}}
\newcommand{\eterm}{\erased{\term}}
\newcommand{\efunc}{\erased{\func}}
\newcommand{\evalue}{\erased{\val}}
\newcommand{\eatvalue}{\erased{\atval}}
\newcommand{\ectxt}{\erased{\ctxt}}

\newcommand{\Expr}{\mathit{Expr}}
\newcommand{\Atom}{\mathit{Atom}}
\newcommand{\Func}{\mathit{Func}}
\newcommand{\Primop}{\mathit{Op}}
\newcommand{\Term}{\mathit{Term}}
\newcommand{\Type}{\mathit{Type}}
\newcommand{\Idx}{\mathit{Idx}}
\newcommand{\Kind}{\mathit{Kind}}
\newcommand{\Sort}{\mathit{Sort}}
\newcommand{\Val}{\mathit{Val}}
\newcommand{\Atval}{\mathit{Atval}}
\newcommand{\Ctxt}{\mathit{Ctxt}}
\newcommand{\wt}[1]{{#1}^{T}}

% Signature, specifying primops' types
\newcommand{\Signature}{\mathcal{S}}
\newcommand{\Sigref}[1]{\Signature{\hskip-.25em}\llb#1\rrb}

% Evaluation context filled with term
\newcommand{\fillc}[2]{#1\hskip-.15em\left[#2\right]}

% Tools for sexp-like things
\newcommand{\parens}[1]{\left( #1 \right)}
\newcommand{\ttparens}[1]{\text{\tt (}#1\text{\tt )}}
\newcommand{\braces}[1]{\left\{ #1 \right\}}
\newcommand{\ttbraces}[1]{\text{\tt \{}#1\text{\tt \}}}
\newcommand{\bracks}[1]{\left[ #1 \right]}
\newcommand{\ttbracks}[1]{\text{\tt [}#1\text{\tt ]}}
\newcommand{\pseq}[1]{\parens{\sequence{#1}}}
% For sexp forms, give the keyword as the first argument and the rest
% of the subexprs as the second argument
\newcommand{\sexp}[2]{\left( #1 \subexp{#2} \right)}
\newcommand{\ttsexp}[2]{\text{\tt(}#1 \subexp{#2}\text{\tt)}}
\newcommand{\ttseq}[1]{\ttsexp{#1}{\text{\tt ...}}}
%\newcommand{\noarg}{\negthickspace}
% If a subexp might be blank, don't necessarily add spacing to separate it
\newcommand{\subexp}[1]{\ifblank{#1}{}{\;#1}}
% Variant for possibly-missing subexp at beginning of list
\newcommand{\subexpcar}[1]{\ifblank{#1}{}{#1\;}}

\let\oldl\l %Save the old \l on \oldl
\newcommand{\cl}{\llap{$\lambda$\hskip-.65em}\phantom{ss}}
%% JFP-friendly versions of \lambda-in-code macros
\renewcommand{\l}[1]{\cl(#1)}
\newcommand{\ttlm}[1]{\cl\ttparens{#1}}
%% Non-JFP versions of \lambda-in-code macros
% \renewcommand{\l}[1]{\ \llap{$\lambda$\hskip-.5em}\ (#1)}
% \newcommand{\ttlm}[1]{\ \llap{$\lambda$\hskip-.5em}\ \ttparens{#1}}

% Syntactic forms
\newcommand{\annotate}[2][]{{#2}^{#1}}
\newcommand{\notevar}[2]{\ttparens{#1 \; #2}}

%\newcommand{\tuple}[2]{\langle #1 , #2 \rangle}
\newcommand{\tuple}[1]{\ttsexp{\text{\tt tuple}}{#1}}
\newcommand{\notedtuple}[2]{\annotate[#1]{\tuple{#2}}}

%\newcommand{\lam}[2]{\parens{\lambda \; \bracks{#1} \; #2}}
\newcommand{\lam}[2]{\ttsexp{\ttlm{#1}}{#2}}
\newcommand{\notedlam}[3][]{\annotate[#1]{\lam{#2}{#3}}}

% \newcommand{\tlam}[2]{
%   \parens{{\tt T\lambda} \bracks{#1} \; #2}}
\newcommand{\tlam}[2]{\ttsexp{{\tt T}\ttlm{#1}}{#2}}
\newcommand{\notedtlam}[3][]{\annotate[#1]{\tlam{#2}{#3}}}

% \newcommand{\ilam}[2]{
%   \parens{{\tt I\lambda} \bracks{#1} \; #2}}
\newcommand{\ilam}[2]{\ttsexp{{\tt I}\ttlm{#1}}{#2}}
\newcommand{\notedilam}[3][]{\annotate[#1]{\ilam{#2}{#3}}}

%\newcommand{\frm}[2]{\text{\tt Frm}\bracks{#1}_{#2}}
%\newcommand{\frm}[2]{\ttsexp{\text{\tt frame}}{\ttparens{#2} \ifblank{#1}{}{\;#1}}}
\newcommand{\frm}[2]{\ttsexp{\text{\tt frame}}{\ttparens{#2} \subexp{#1}}}
\newcommand{\notedfrm}[3][]{\annotate[#1]{\frm{#2}{#3}}}

%\newcommand{\emptyfrm}[2]{\text{\tt Frm}^{#1}_{#2}}
\newcommand{\emptyfrm}[2]{\ttsexp{\text{\tt frame}}{\ttparens{#2} \subexp{#1}}}
\newcommand{\notedemptyfrm}[3][]{\annotate[#1]{\frm{#2}{#3}}}

%\newcommand{\arrlit}[2]{\text{\tt Arr}\bracks{#1}_{#2}}
\newcommand{\arrlit}[2]{\ttsexp{\text{\tt array}}{\ttparens{#2} \subexp{#1}}}
\newcommand{\notedarrlit}[3][]{\annotate[#1]{\arrlit{#2}{#3}}}

\newcommand{\emptyarrlit}[2]{\ttsexp{\text{\tt array}}{\ttparens{#2} \subexp{#1}}}
\newcommand{\notedemptyarrlit}[3][]{\annotate[#1]{\frm{#2}{#3}}}

%\newcommand{\app}[2]{\parens{#1 \; #2}}
\newcommand{\app}[2]{\ttsexp{#1}{#2}}
\newcommand{\notedapp}[3][]{\annotate[#1]{\app{#2}{#3}}}

%\newcommand{\tapp}[2]{\parens{\text{\tt T-APP} \; #1 \; #2}}
\newcommand{\tapp}[2]{\ttsexp{\text{\tt t-app}}{#1 \subexp{#2}}}
\newcommand{\notedtapp}[3][]{\annotate[#1]{\tapp{#2}{#3}}}

\newcommand{\iapp}[2]{\ttsexp{\text{\tt i-app}}{#1 \subexp{#2}}}
\newcommand{\notediapp}[3][]{\annotate[#1]{\iapp{#2}{#3}}}

%\newcommand{\dsum}[3]{\parens{ \text{\tt box} \; #1 \; #2 \; : #3 }}
\newcommand{\dsum}[3]{\ttsexp{\text{\tt box}}{#1 \subexp{#2} \subexp{#3}}}
\newcommand{\noteddsum}[3][]{
  \annotate[#1]{
    \ttsexp{ \text{\tt box} \subexp{#2} \subexp{#3}}}}

\newcommand{\dproj}[4]{
  \ttsexp
  {\text{\tt unbox}}
  % Typesetting this is weird because the "optional" piece is #1, so its
  % trailing space should be guarded by \ifblank{#1}, rather than considering it
  % attached to #2
  {\ttparens{\subexpcar{#1}#2 \subexp{#3}} \subexp{#4}}}
\newcommand{\noteddproj}[5][]{\annotate[#1]{\dproj{#2}{#3}{#4}{#5}}}

\newcommand{\typefun}[2]{\ttsexp{\text{\tt ->}}{\ttparens{#1} \; #2}}
%{\ttsexp{#1}{\text{\tt ->} \; #2}}
\newcommand{\typeprod}[2]{\ttsexp{\text{\tt Tuple}}{#1 \; #2}}
\newcommand{\typeuniv}[2]{\ttsexp{\text{\tt Forall}}{\ttparens{#1} \; #2}}
\newcommand{\typedprod}[2]{\ttsexp{\text{\tt Pi}}{\ttparens{#1} \; #2}}
\newcommand{\typedsum}[2]{\ttsexp{\text{\tt Sigma}}{\ttparens{#1} \; #2}}
%\newcommand{\typearray}[2]{#1 #2}
\newcommand{\typearray}[2]{\ttsexp{\text{\tt Arr}}{#1 \; #2}}

\newcommand{\idxshape}[1]{\ttsexp{\text{\tt Shp}}{#1}}
\newcommand{\idxadd}[1]{\ttsexp{\text{\tt +}}{#1}}
\newcommand{\idxappend}[1]{\ttsexp{\text{\tt ++}}{#1}}
%\newcommand{\idxappend}[1]{\braces{\thappend \; #1}}

\newcommand{\kindarray}{\text{\tt Array}}
\newcommand{\kindatom}{\text{\tt Atom}}

\newcommand{\sortdim}{\text{\tt Dim}}
\newcommand{\sortshp}{\text{\tt Shape}}


% Judgment forms
\newcommand{\rulename}[1]{\quad \textsc{#1}}
\newcommand{\seqpremise}[2]{#2 \; \; \text{for each $#1$}}

\newcommand{\hassort}[2]{#1 :: #2}
\newcommand{\sortof}[3]{#1 \vdash \hassort{#2}{#3}}

\newcommand{\haskind}[2]{#1 :: #2}
\newcommand{\kindof}[4]{#1;#2 \vdash \haskind{#3}{#4}}

\newcommand{\hastype}[2]{#1 : #2}
\newcommand{\typeof}[5]{#1;#2;#3 \vdash \hastype{#4}{#5}}

\newcommand{\typeeqsym}{\cong}
\newcommand{\teqv}[2]{#1 \typeeqsym #2}
\newcommand{\ieqv}[2]{\text{\sc Valid} \llb #1 \theq #2 \rrb}

\newcommand{\wfenv}[3]{#1 ; #2 \vdash #3}

\newcommand{\fresh}[1]{\quad\text{with fresh $#1$}}


% "Replace Y with Z"
\newcommand{\singlesubst}[2]{#1 \mapsto #2}
% "In X, replace ____"
\newcommand{\multisubst}[2]{#1\hspace{-2pt}\bracks{#2}}
% "In X, replace Y with Z
\newcommand{\subst}[3]{\multisubst{#1}{\singlesubst{#2}{#3}}}
% "In X, replace Ys with Zs"
\newcommand{\seqsubst}[3]{\multisubst{#1}{\sequence{\singlesubst{#2}{#3},}}}


% Evaluation rules
\newcommand{\evalrule}[4][]{
  \mbox{
    \begin{tabular}{l}
       #2 \\ $ \; \mapsto_{\mathit{#1}} $ #3
    \end{tabular}
  }\\
  \mbox{#4}
}
\newcommand{\rulesep}{\medskip\\}
\newcommand{\0}{\hspace*{0em} }


% Proof utilities
\newcommand{\pfstub}{{\color{red} Left as an exercise for the author}}
\newcommand{\cfitem}[4][]{
\item{
  If $\type$ is of the form $#3$,\\
  then $#2$ is of the form $#4$#1.}
}
\newcommand{\cfarritem}[4][]{
  \cfitem
      [#1]
      {#2}
      {\typearray{#3}{\idx}}
      {\arrlit{\sequence{#4}}{\sequence{\nat}}}}

% "Collapsible" proof environment: give \pfskip as argument to elide the proof
\newcommand{\pfskip}[1]{{\color{cyan} elided for editing}}
\NewEnviron{cproof}[1][]{\begin{proof}#1{\BODY}\end{proof}}
% "Sketchable" proof environment: consults \pftype to pick version of proof
% (can select \fullproof or \sketchproof or \collapseproof)
\def\fullproof{0}
\def\sketchproof{1}
\def\collapseproof{2}
\NewEnviron{sproof}[1][{\color{magenta} sketch missing}]
{\begin{proof}
\if\pftype\fullproof {\BODY} \else\if\pftype\sketchproof #1 \else \pfskip{} \fi\fi
\end{proof}}
\newcommand{\TODO}{{\color{red} [TODO]}}

% Gadgets for sketching judgment derivations
\newcommand{\somehow}[1]{\inferrule*{\vdots}{#1}}
\newcommand{\teqvInd}[2]{\somehow{\teqv{#1}{#2}}}
\newcommand{\typeofInd}[5]{\somehow{\typeof{#1}{#2}{#3}{#4}{#5}}}
\newcommand{\kindofInd}[4]{\somehow{\kindof{#1}{#2}{#3}{#4}}}
\newcommand{\sortofInd}[3]{\somehow{\sortof{#1}{#2}{#3}}}
\newcommand{\infr}[3][]{\inferrule*[right=\;#1]{#2}{#3}}
\newcommand{\ctrand}{\[\text{and}\]}

% Erasure functions and related things
\newcommand{\EraseE}[1]{\mathcal{E}{\hskip-.25em}\llb #1 \rrb}
\newcommand{\EraseA}[1]{\mathcal{A}{\hskip-.25em}\llb #1 \rrb}
\newcommand{\EraseT}[1]{\mathcal{T}{\hskip-.25em}\llb #1 \rrb}
\newcommand{\EraseC}[1]{\mathcal{C}{\hskip-.25em}\llb #1 \rrb}
\newcommand{\EraseTrm}[1]{\mathcal{R}{\hskip-.25em}\llb #1 \rrb}
\newcommand{\EraseEqv}{\cong_{\mathcal{E}}}

%% What you frequently want when you say \tt:
\def\ttt{\ttfamily\upshape\mdseries\catcode``=13\@noligs\frenchspacing}

%% Centered version of alltt environment
\newenvironment{centertt}{%
  \par\medskip
  \centering
  \varwidth{\linewidth}%
  \alltt
}{%
  \endalltt
  \endvarwidth
  \vspace{-5pt}
  \par
}

% Works in math mode; all special chars remain special; cheaper than \cd.
% Will not be correct size in super and subscripts, though.
\newcommand{\ex}[1]{\mbox{\ttt{#1}}}

\newenvironment{inset}
 {\bgroup\parskip=1ex plus 1ex\begin{list}{}%
        {\topsep=0pt\rightmargin\leftmargin}%
        \item[]}%
 {\end{list}\leavevmode\egroup\global\@ignoretrue}

\newenvironment{tightinset}
 {\bgroup\parskip=0pt\begin{list}{}%
        {\topsep=0pt\rightmargin\leftmargin}%
        \item[]}%
 {\end{list}\leavevmode\egroup\ignorespaces}

\newenvironment{leftinset}
 {\bgroup\parskip=1ex plus 1ex\begin{list}{}%
        {\topsep=0pt}%
        \item[]}%
 {\end{list}\leavevmode\egroup\global\@ignoretrue}

% For typesetting interactive examples.
\newcommand{\result}[1]{\textsl{#1}}

% For multiletter vars in math mode:
\renewcommand{\v}[1]{\ensuremath{\mathit{#1}}} % \frenchspacing?
\newcommand{\vi}[2]{\ensuremath{\mathit{#1}_{#2}}}

\newcommand{\tu}{\ensuremath{\rightarrow}}

\newcommand{\ft}[2]{(\tu\ (#1) #2)}
\newcommand{\faty}[2]{(\(\forall\) (#1) {#2})}
\newcommand{\pity}[2]{(\(\Pi\) (#1) {#2})}
\newcommand{\vari}[2]{\ensuremath{#1_{#2}}}

\makeatother

